REALM: RAG-Driven Enhancement of Multimodal Electronic Health Records Analysis via Large Language Models

The integration of multimodal Electronic Health Records (EHR) data has significantly improved clinical predictive capabilities. Leveraging clinical notes and multivariate time-series EHR, existing models often lack the medical context relevent to clinical tasks, prompting the incorporation of external knowledge, particularly from the knowledge graph (KG). Previous approaches with KG knowledge have primarily focused on structured knowledge extraction, neglecting unstructured data modalities and semantic high dimensional medical knowledge. In response, we propose REALM, a Retrieval-Augmented Generation (RAG) driven framework to enhance multimodal EHR representations that address these limitations. Firstly, we apply Large Language Model (LLM) to encode long context clinical notes and GRU model to encode time-series EHR data. Secondly, we prompt LLM to extract task-relevant medical entities and match entities in professionally labeled external knowledge graph (PrimeKG) with corresponding medical knowledge. By matching and aligning with clinical standards, our framework eliminates hallucinations and ensures consistency. Lastly, we propose an adaptive multimodal fusion network to integrate extracted knowledge with multimodal EHR data. Our extensive experiments on MIMIC-III mortality and readmission tasks showcase the superior performance of our REALM framework over baselines, emphasizing the effectiveness of each module. REALM framework contributes to refining the use of multimodal EHR data in healthcare and bridging the gap with nuanced medical context essential for informed clinical predictions.

==> sections/methods.tex <==

在进行病历样本分类任务时，仅仅依靠未经处理过的病历信息无法使模型精确的对病人情况进行分类。医疗图谱将疾病和症状的属性以三元组格式存放，每一个疾病和症状类型中有很多属性信息，用于补充对疾病和症状的说明，可以作为检索文献来补充病历中的相关信息，为模型判断提供更多的特征依据。为了完成对病历样本的准确分类任务，本文使用一种向量检索增强的方法进行优化，源数据是病人病历内容，经过特征提取后在医疗图谱作为文献进行检索匹配，具体进行了如下的迭代实验：——放在method，陈述KG的motivation

第一步：由于病历文本内容过长，存在大量对分类无意义的数据，使用医疗领域预训练模型（bert or LLM）进行关键实体抽取，从病历中获取疾病和症状的相关名词信息，将病历中抽取的实体作为在医疗图谱中检索的关键字输入，经过匹配后，依据相关性（需要补充RAG方法）选择关联文本一同进行编码，最后使用分类器对包含特征的编码内容进行二分类，得到分类结果；（需不需要给出这一步实验结果）——放在method

第二步：在第一步中，仅仅使用实体关键词进行匹配，并不能代表病历中的全部内容，可能会由于信息不全导致一些误报（举一个例子？），因此在第二轮迭代中，将实体抽取出的关键词重新放入病历中进行匹配，做上下文补全，充实疾病和症状的相关信息，明确所在部分的主要语义，将补全后的上下文输入医疗图谱中进行检索，得到一个和病历信息更为贴合的召回结果，在进行编码和分类，从结果来看这种优化使分类结果更加准确；（补充实验结果）——放在ablation  study

第三步：向量检索模型的优化，尝试使用小量级模型bge-base、bge-m3和大语言模型qwen、baichuan进行文本向量化获得特征向量，然后进行相似匹配做向量检索增强，测试对分类结果如下（列出测试结果表格）。

第四步：编码方法的优化，基于关键词和上下文在医疗图谱中将相关文本召回后，使用语言模型进行编码（不知道理解的对不对），由于病人病情是随着时间不断变化的，因此在编码时按照时间步分开编码能够显著提示分类的准确度。

